Stochastic Block Model and Community Detection in the Sparse Graphs: A spectral algorithm with optimal rate of recovery

In this paper, we present and analyze a simple and robust spectral algorithm for the stochastic block model with $k$ blocks, for any $k$ fixed. Our algorithm works with graphs having constant edge density, under an optimal condition on the gap between the density inside a block and the density between the blocks. As a co-product, we settle an open question posed by Abbe et. al. concerning censor block models.

==> improvedClustering.tex <==
By a simple application of Chernoff bound, we have
\begin{lemma}
With probability at least $1- o(1)$, at least $m/2$ of the vectors $\ee_1,...,\ee_m$ satisfy $$ \nbr{P_{W} \ee_i} < 2 \sigma k^{1/2} .$$
\end{lemma}

%Since the events that $ \nbr{P_{W} \ee_i} < 2 \sigma k^{1/2} $ are independent for $i=1,...,m$, we know that of the $m=2 \log n$ columns, a uniformly random subset of size at least $\log n$ satisfy the condition.  
We call a vector $\bb_i$ good if the corresponding vector $\ee_i$ satisfies 
$$\nbr{P_{W} \ee_i} < 2 \sigma k^{1/2}.$$
Every good vector $\bb_i$ gives us a $0.1$-correct cluster. 

We now argue that we can detect which $\bb_i$ gives a good cluster by looking at the edge density.

\begin{lemma}
There exists a constant $c>0$ such that the following holds. Suppose we are given a set $X \subset Y_2$ of size $|X| = n/4$. If for all $i \in {1,...,k}$  $$|X \cap V_{i}| \le 0.9 |X|,$$ then with probability at least $1 - e^{-cn}$  the number of RED edges in the graph induced by $X$ is at most $an/32 - 0.09(a-b)n/32$. Conversely, if $$|X \cap V_{i}| \ge 0.95 |X|$$ for some $i \in {1,...,k}$, then with with probability at least $1 - e^{-cn}$ the number of RED edges in the graph induced by $X$ is at least $an/32 - 0.09(a-b)n/32.$
\end{lemma}

\proof

Let $e(X)$ denote the number of RED edges in the graph induced by vertices in $X$. Suppose $|X \cap V_{i}| \le 0.9 |X|$ for all $i \in {1,...,k}$.  Then 
$$\E e(X) \le an/32 - 0.09(a-b)n/16.$$
To bound the probability that $\E e(X) \ge an/32 - .045(a-b)n/16$, we can use Chernoff bound. Let $\delta = \frac{0.045(a-b)n/16}{an/32 - 0.09(a-b)n/16}.$
$$\mathbb{P}(\E e(X) \ge an/32 - .045(a-b)n/16) \le \exp \left( -\frac{(.045(a-b)n/16)^2}{2an/32+0.045(a-b)n/16} \right).$$

Similarly, suppose $|X \cap V_{i}| \ge 0.95 |X|$ for some $i \in {1,...,k}$.  Then 
$$\E e(X) \ge an/32 - 0.05(a-b)n/32.$$
To bound the probability that $\E e(X) \le an/32 - .045(a-b)n/16$, we can use Chernoff bound. Let $\delta = \frac{0.04(a-b)n/32}{an/32 - 0.05(a-b)n/32}.$
$$\mathbb{P}(\E e(X) \le an/32 - .045(a-b)n/16) \le \exp \left( -\frac{(.04(a-b)n/32)^2}{2an/32+0.04(a-b)n/32} \right).$$

